Equalized odds postprocessing under imperfect group information

Most approaches aiming to ensure a model's fairness with respect to a protected attribute (such as gender or race) assume to know the true value of the attribute for every data point. In this paper, we ask to what extent fairness interventions can be effective even when only imperfect information about the protected attribute is available. In particular, we study the prominent equalized odds postprocessing method of Hardt et al. (2016) under a perturbation of the attribute. We identify conditions on the perturbation that guarantee that the bias of a classifier is reduced even by running equalized odds with the perturbed attribute. We also study the error of the resulting classifier. We empirically observe that under our identified conditions most often the error does not suffer from a perturbation of the protected attribute. For a special case, we formally prove this observation to be true.

==> related_work.tex <==
\section{RELATED WORK}\label{section_related_work}


By now, there is a huge body of work on fairness in 
ML, 
mainly  in supervised learning 
%could add: Kamiran2012
\citep[e.g.,][]{Kamishima2012,zemel2013,feldman2015,hardt2016equality,kleinberg2017,pleiss2017,woodworth2017,
zafar2017,zafar2017www,agarwal2018,donini2018,menon2018,FairGAN2018,kallus2019}, 
but 
more 
recently also in  unsupervised learning  
%could add: samira2019
\citep[e.g.,][]{fair_clustering_Nips2017,celis2018,sohler_kmeans,samira2018,fair_k_center_2019,fair_SC_2019}. 
All of these papers assume to know the true value of the protected attribute for each data point. We will discuss some papers not making this assumption below. 
First we discuss the pieces of work
 related to the fairness notion of equalized odds, which is central to our paper and one of the most prominent fairness notions in the ML literature
 (see \citealp{Verma2018}, for a 
 summary of the various 
 notions and a citation~count).
%
 

 
% \paragraph{Equalized Odds}
 \vspace{3mm}
 \textbf{Equalized Odds~~}
 Our paper builds upon the equalized odds postprocessing method of \citet{hardt2016equality} as described in Section~\ref{section_equalized_odds_MAIN}. 
\citeauthor{hardt2016equality} also show how to derive an optimal predictor
satisfying
the equalized odds criterion based on a biased score function
%~$S$  
%(with values in $[0,1]$ expressing the likelihood of $Y=1$) 
rather than a binary classifier $\widetilde{Y}$. 
However, in this case the resulting optimization problem is no longer a linear program and it is unclear how to 
extend 
our analysis to it. 
%
Concurrently with 
the paper by 
\citeauthor{hardt2016equality}, the fairness notion of equalized odds has also been proposed by \citet{zafar2017www} under the name of disparate mistreatment. 
\citeauthor{zafar2017www} incorporate a proxy for the equalized odds criterion into the training phase of a decision boundary-based classifier, 
which leads to a convex-concave optimization problem and does not come with any theoretical guarantees.
%
 \citet{kleinberg2017} prove that, except for trivial cases, a classifier cannot satisfy the equalized odds criterion and the fairness notion of 
 calibration within groups 
 %\citep{kleinberg2017} 
 at the same time. Subsequently,  \citet{pleiss2017} show how to achieve calibration within groups and  a relaxed 
 form of the equalized odds constraints 
 %at the same time.
 simultaneously. 
 \citet{woodworth2017} show that 
 %for certain loss functions 
 postprocessing a Bayes optimal 
 %unfair 
 classifier does not necessarily lead to a Bayes optimal fair classifier (fair 
 %/ unfair 
 with respect to the 
 %fairness 
 notion of equalized odds).  
 They propose a two stage procedure where some approximate fairness constraints are incorporated into the empirical risk minimization framework to get a classifier that 
 is fair to a non-trivial degree, and then using the equalized odds postprocessing method of \citeauthor{hardt2016equality} to get the final classifier. 
 %
 We also want to mention the critical work of \citet{corbett_davies_goel_2018}, which points out some limitations of 
  prominent 
  group fairness notions, 
  including 
 %the fairness notion of 
 equalized~odds.  
 

 
 
 
 
\begin{figure*}[t]
 \centering
\includegraphics[width=7.1cm]{{Experiments/Simulations/Bal_and_error_a1=0.9_b1=0.8_a2=0.4_b2=0.1_ChoiceG=0_NoLegend}.pdf}
\hspace{8mm}
\includegraphics[width=7.1cm]{{Experiments/Simulations/Bal_and_error_a1=0.9_b1=0.6_a2=0.7_b2=0.1_ChoiceG=2_GOOD_LEGEND}.pdf}

\vspace{3mm}
\includegraphics[width=7.1cm]{{Experiments/Simulations/Bal_and_error_a1=0.9_b1=0.6_a2=0.4_b2=0.1_ChoiceG=0_NoLegend}.pdf}
\hspace{8mm}
\includegraphics[width=7.1cm]{{Experiments/Simulations/Bal_and_error_a1=0.9_b1=0.6_a2=0.3_b2=0.8_ChoiceG=1_NoLegend}.pdf}
\caption{$\Bias_{Y=1}(\widehat{Y})$ (dashed blue) and $\Error(\widehat{Y})$ (dashed red) as a function of the perturbation level for various choices of the problem parameters 
(see the titles of the plots and Table~\ref{table_parameters_main} in Appendix~\ref{subsec_table1}). 
For $\gamma_{1,0}=0$ it is $\widehat{Y}=\Ytrue$, and for $\gamma_{1,0}>0$ it is $\widehat{Y}=\Ycorr$.
The solid lines show the bias (blue) and the error (red) of the given predictor~$\widetilde{Y}$. The dotted cyan 
curve shows the bound on $\Bias_{Y=1}(\widehat{Y})$ provided in \eqref{theorem_bias_formula} in Theorem~\ref{theorem_bias}. 
%Note that 
In the right bottom plot, 
Assumption~\ref{assu_error} is not satisfied and here the error of $\widehat{Y}$ initially increases, that is \eqref{claim_error} does not hold.}\label{figure_simulations}
\end{figure*}


 

 
 
 
 
%\paragraph{Fairness without Protected Attributes} 
\vspace{3mm}
\textbf{Fairness without Protected Attributes} 
\citet{fta2012} phrased the notion of individual fairness 
%already 
mentioned in Section~\ref{section_intro}, 
according to which similar data points (as measured by a given metric) should be 
treated similarly by a randomized classifier. 
%
Only recently, there have been works studying how to satisfy group fairness criteria when having only limited information about the protected attribute. 
%
Most important to mention are  the 
works by  \citet{gupta2018} and \citet{lamy2019}. 
%The paper of 
\citet{gupta2018} empirically show that 
when the protected attribute is not known, improving a fairness metric  
for a proxy of the true 
%protected 
attribute 
%might be a valuable strategy to 
can 
improve the fairness metric for the true attribute. 
Our paper provides theoretical evidence 
for their observations.
%
\citet{lamy2019} study a scenario related to ours and consider training a fair classifier when the 
protected  attribute is corrupted 
according to a mutually contaminated model \citep{scott2013}. 
In their case, 
%``training'' 
training 
is done by means of constrained empirical risk minimization 
and requires to solve a non-convex optimization problem. 
Similarly to our Theorem~\ref{theorem_bias}, they show that the bias  of a classifier trained with the corrupted 
attribute grows in a certain way with the amount of corruption (where the bias is defined according to the fairness notions of equalized odds or demographic parity). 
However, they do not  
investigate the error 
of such a classifier. 
Importantly, \citeauthor{lamy2019} only consider classifiers that do not use the protected attribute when making a prediction 
for 
%the ground-truth label of 
a test point and pose it as an open question to extend their results to classifiers that do use the 
%protected 
attribute 
%when making a prediction. 
in the test phase. 
% In our paper, we study the bias \emph{and} the error of a derived equalized odds predictor under a perturbation of the protected attribute 
% in the training phase of the equalized odds 
% %postprocessing 
% method. 
Since 
a derived equalized odds predictor crucially depends on the protected attribute when making a prediction in the test phase, 
our paper addresses 
%the question raised by \citeauthor{lamy2019}.
their question. 
%
%Next, 
%\citet{Hashimoto2018} 
Also important to mention is the paper by \citet{Hashimoto2018}, 
which
%It
uses distributionally robust optimization in order to minimize the worst-case misclassification risk in a $\chi^2$-ball around the data generating distribution. 
In doing so, under the assumption that the resulting non-convex optimization problem was solved exactly, 
one provably 
controls the risk of each protected group without knowing which group a data point belongs to. \citeauthor{Hashimoto2018} also show that their approach helps to avoid disparity amplification 
in a sequential classification setting in which a group's fraction in the data decreases as its misclassification risk increases. 
As an application of our results, in Section~\ref{subsec_exp_repeated_loss_minimization} /  Appendix~\ref{supp_mat_rep_loss_min}  
%and Appendix~\ref{supp_mat_rep_loss_min}, respectively, 
we experimentally compare the approach of \citeauthor{Hashimoto2018} to the 
equalized odds method with perturbed 
%protected 
attribute information in such a sequential setting.  
%
There are a couple of more works that we want to discuss. 
\citet{botros2018} propose a variational autoencoder for learning fair representations \citep{zemel2013,louizos2016} that also works when the protected attribute is only partially 
%(i.e., for only some of the data points)
observed.   
%
%The paper by 
\citet{kilbertus2018} provide an approach to fair classification when users to be classified are not willing to share their protected attribute but only
an encrypted version of it. 
Their approach assumes the existence of a regulator with fairness aims and is based on secure multi-party computation.  
%
\citet{chen_fairness_under_unawareness} study the problem of assessing the demographic disparity of a classifier when the protected attribute is 
unknown and has to be estimated from data.  
%
%Finally, 
\citet{coston2019} study
%the problem of 
fair classification in a covariate shift setting where the 
%protected 
attribute is  
only available in the source domain but not in the target domain (or the other way round). 
%
Finally, we want to mention the recent line of work on 
%the notion of 
\emph{rich subgroup fairness} \citep{Hebert2018,kearns_2018_subgroup1,kearns_2018_subgroup2}.
%which 
%in a way 
This notion 
falls between the categories of individual and group fairness in that it requires some statistic to be similar 
for a \emph{large} (or even infinite) number of subgroups,  
which are 
%of the population. In contrast to our setting, subgroups are not defined via a single protected attribute, but 
defined 
via a function class.
%, and 
%
%
% The cited papers 
% relate properties of the resulting fairness problem to the learnability of the function~class. Some of these works do not explicitly require the knowledge
% of the sensitive attribute information if given query access to human auditors. Our goal is orthogonal and is trying to characterize noise sensitivity of an existing 
% popular algorithm, rather than proposing a new one or changing the interaction model.
% %
% \textcolor{orange}{Pranjal: please add a sentence here highlighting the benefits of our paper.}
% 
% 
% \textcolor{red}{Can you verify the last paragraph on subgroupfairness? I only mention it because one Neurips reviewer wrote 
% ``One line of work that is worth comparing to is the line of work on
% subgroup fairness. ... In these works, they don't need an explicit notion of protected
% attribute because they instead learn subpopulations that need adjustment. In this setting, as long as their auditors are
% sufficiently expressive to capture (correlate with) the sensitive attribute, then no explicit dependence on the sensitive
% attribute is necessary.'' It's not clear to me how to deal with his last sentence.}
% 

